RACECAR -- The Dataset for High-Speed Autonomous Racing

This paper describes the first open dataset for full-scale and high-speed autonomous racing. Multi-modal sensor data has been collected from fully autonomous Indy race cars operating at speeds of up to 170 mph (273 kph). Six teams who raced in the Indy Autonomous Challenge have contributed to this dataset. The dataset spans 11 interesting racing scenarios across two race tracks which include solo laps, multi-agent laps, overtaking situations, high-accelerations, banked tracks, obstacle avoidance, pit entry and exit at different speeds. The dataset contains data from 27 racing sessions across the 11 scenarios with over 6.5 hours of sensor data recorded from the track. The data is organized and released in both ROS2 and nuScenes format. We have also developed the ROS2-to-nuScenes conversion library to achieve this. The RACECAR data is unique because of the high-speed environment of autonomous racing. We present several benchmark problems on localization, object detection and tracking (LiDAR, Radar, and Camera), and mapping using the RACECAR data to explore issues that arise at the limits of operation of the vehicle.

==> acknowledgements.tex <==
We would like to thank all contributors towards the data collection, parsing, and schema generation. 

==> data_acquisition.tex <==


Nine AV-21 racecars outfitted with a full autonomous sensor suite were built for teams participating in the Indy Autonomous Challenge \cite{iac}, a competition to race these autonomous vehicles at high speed. 
The Indy challenge possessed a \$ 1 million prize, and was awarded to the team to run the fastest laps at the Indianapolis Motor Speedway. 
A subsequent challenge was held at CES in Las Vegas, at the Las Vegas Motor Speedway. 

The competition evolved and teams participated in a head to head passing competition, with two cars on track at a time. 
All nine vehicles were outfitted with the same vehicle setup and sensor specifications, 


==> data_conversion.tex <==
The \texttt{rosbag2nuscenes} library was developed to convert the data originally stored in ROS2 bag files to the nuScenes format. 
An overview of the conversion process is shown in Figure \ref{fig:nuscenes_conversion}. 
Using the rosbag2 Python API, the conversion library reads through the database entries in chronological order and extracts the necessary ROS2 messages specified in a separate parameter file. 
Entries are first created in the JSON files that store information about the context of the scene and the calibration of the vehicle's sensors. 
The odometry data of the ego vehicle in global coordinates is then converted into a nuScenes formatted JSON file, followed by each of the perception sensors. 
As entries are populated in the appropriate JSON files, the library generates unique tokens to establish links between entries.
%The dataset created by the conversion tool improves upon the original nuScenes format by writing all JSON entries in chronological order, making the dataset easier to inspect while still maintaining compatibility with existing tools for developing with nuScenes formatted data. 
The sampling rate is set at the default rate of 2 Hz, but is also adjustable for each scene, as laps at higher speeds warrant higher sampling rates than those at lower speeds. Lastly, scenes also last significantly longer than the twenty second clips in the original nuScenes dataset and contain repeated laps around the track. 
This leaves potential for testing localization algorithms, such as SLAM, discussed more in Section~\ref{sec:benchmarks}.
% The library and documentation will also be released on the RACECAR Github (link withheld due to double blind review).

==> data_description.tex <==
data description (candidate bags, number of scenes)

==> dataset_content.tex <==
The participating six multi-agent capable racing teams provided rosbag2 data for several selected driving scenarios \ref{tab:drivingscenarios}, with varying coverage in sensor modality \ref{tab:Dataset}. All teams provided GNSS coordinate information, which has been converted into a common local coordinate system. These local coordinates have been used to provide ground truth information for opposing vehicle's position and heading. How this ground truth information can help supplement use of the perception data will be further discussed in \ref{sec:benchmarks}.

For the positioning of each sensor, a full Unified Robot Description Format (URDF) is provided. This supplies appropriate transforms for each sensor with respect to the base link of the vehicle.





==> driving_environment.tex <==
% \begin{figure}
%   \centering 
%   \includegraphics[width=\columnwidth]{images/tracks_single_column}
%   \caption{AV-21 avoiding a pylon at Indianapolis Motor Speedway, and completeing an overtake maneuver at Las Vegas Motor Speedway}\label{fig:scenarios}
% \end{figure}



\begin{table*}
\centering
\begin{tabular}[c]{ ||p{5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}||}
 \hline
 \textbf{Scenario (Teams)}  & \textbf{GNSS} & \textbf{LiDAR} & \textbf{RADAR} & \textbf{Camera}   \\
 \hline
 $S_{1} (C, M, P)$ & 51,486 & 58,375 & 9,924 & 157,146 \\
 \hline
 $S_{2} (C, M, K)$ & \checkmark & \checkmark & \checkmark & \checkmark \\
 \hline
 $S_{3} (M, E)$ & \checkmark & \checkmark & \checkmark & \checkmark \\
 \hline
 $S_{4} (T, E)$ & \checkmark & \checkmark & \checkmark & \checkmark \\
 \hline
 $S_{5} (C, M, P, T, E, K)$ & \checkmark & \checkmark & \checkmark & \checkmark \\
 \hline
 $S_{6} (T, E, P)$ & \checkmark & \checkmark & \checkmark & \\
 \hline
 $S_{7} (C, K)$ & \checkmark & \checkmark & & \\
 \hline
 $S_{8} (C, K)$ & \checkmark & \checkmark & & \\
 \hline
 $S_{9} (T, E)$ & \checkmark & \checkmark & & \\
 \hline
 $S_{10} (P)$ & \checkmark & \checkmark & & \\
 \hline
 $S_{11} (T, K)$ & 22,594 & 29,746 & 6,440 & 278,009 \\
 \hline
\end{tabular}
\caption{Dataset Content: Will include frame counts after data analysis}
\label{tab:Dataset}
\end{table*}

  The AV-21s ran at two racetracks, the Indianapolis Motor Speedway and the Las Vegas Motor Speedway.
The Indianapolis Motor Speedway (IMS) is a 2.5 mile symmetric oval loop, possessing long flat straights and 9 degree banking on turns.
Vehicles ran individually at IMS, attempting high speed solo runs and static obstacle avoidance.
The Las Vegas Motor Speedway (LVMS) is a shorter 1.5 mile asymmetric oval loop. 
There is a consistent 12 degree bank throughout the track that progressively transitions to 20 degrees on turns.
This variation in banking provides a unique environment where the autonomous vehicle is travelling at an angle with respect to the inner bounds of the track.
At Vegas, cars ran in both time trials or in head-to-head racing.
The racecar would be exiting or entering pitlane, transitioning onto the main track, driving around the respective oval tracks alone, or in head-to-head racing with another car. 
The various racing scenes are described in Table \ref{tab:drivingscenarios}.
For both tracks, vehicles were run only during daylight as well as in racing conditions (not too cold and no rain) for safety considerations.


==> networking.tex <==
All sensors except Radars were connected to a Cisco IE5000 Switch and interfaced with in an ADLINK computer. 
Radars were connected directly to a CAN bus on the ADLINK. Some sensor data was networked using either 40 GbE QSFP connections, or GigE RJ45 ports. 
Sensor data was written to either NVME or SATA connected hard drives, resulting in varying sensor capture rate relative to data processing rate.
The switch is capable of acting as a Global Master clock for time synchronization between all device clocks other than Radar using Precision Time Protocol. 

==> racecar_setup.tex <==






